The first IXPE view of the eclipsing ADC source 4U 1822-37

Accretion-disc corona sources are high-inclination low-mass X-ray binaries in which the innermost regions are hidden and the observed X-ray emission is dominated by radiation scattered above the disc. 4U 1822-37 is a key binary system of this class, but its geometry is still debated. X-ray polarimetry offers a direct probe of the scattering structure. We present the first X-ray spectro-polarimetric study of 4U 1822-37 and test whether its spectrum and polarisation can be explained within the accretion-disc-corona scenario. We analysed a coordinated campaign with IXPE, XMM-Newton, NuSTAR, and Swift. We performed broadband spectral modelling and model-independent, energy-resolved, and orbital-phase-resolved polarimetric analyses. The broadband spectrum requires a soft thermal component, a Comptonised continuum, a hard power-law tail, and relativistically blurred reflection. The observed 0.1-100 keV luminosity, $L_{\rm obs}\simeq6.1\times10^{36}\ {\rm erg\,s^{-1}}$, is far below the intrinsic luminosity expected from the orbital evolution, supporting a geometry in which only a small fraction of the intrinsic emission is scattered into the line of sight by an extended, optically thin corona. In the 2-8 keV band, IXPE measures ${\rm PD}=7.9\pm0.6\%$ and ${\rm PA}=-24^\circ\pm2^\circ$. The PD increases with energy, while the PA remains approximately constant. During eclipse, the PD decreases to ${\rm PD}=5.5\pm1.7\%$, with no significant PA variation. This behaviour is consistent with the companion occulting the most polarimetrically efficient part of the extended corona. The high PD, stable PA, energy-dependent polarisation, and eclipse behaviour support a picture in which 4U 1822-37 is observed in an extreme high-inclination, scattering-dominated regime. The extended corona is the main structure shaping both the observed X-ray emission and its polarisation.

==> appunti.tex <==
La prima cosa forte è il confronto globale tra polconst su tutto e pollin su tutto. Qui il messaggio è pulito: con la DU2 inclusa la polarizzazione totale non solo resta alta, ma la descrizione con una PD crescente con l’energia è preferita in modo significativo rispetto a una costante. Il fatto che la slope della PA sia compatibile con zero mentre quella della PD no è esattamente il comportamento che ci aspettavamo già guardando i punti: l’orientazione del vettore polarizzato resta stabile, mentre la sua ampiezza cresce con l’energia. Questo, per me, è il risultato osservativo più robusto di tutta la sezione spettro-polarimetrica. È anche quello che va messo davanti a tutto, perché è il meno dipendente dalle assunzioni sui singoli componenti.

Quando poi passi alla scomposizione in componenti, la situazione diventa inevitabilmente più degenerata. E questo si vede subito nei modelli con due polconst: il fit è peggiore del caso globale e, soprattutto, la reflection non è davvero ben vincolata. Che tu lasci gli angoli separati o li leghi, il risultato quasi non cambia, e la PA della componente dominante resta sempre attorno a -23^\circ / -26^\circ, cioè molto vicina alla PA totale. Questo ti dice una cosa importante: il segnale osservato è dominato dalla componente continua, mentre la reflection contribuisce ma non sta imponendo da sola la geometria del vettore totale.

Il confronto davvero interessante è quello tra il caso a componenti costanti e il caso a componenti crescenti. Lì si vede che introdurre una dipendenza lineare migliora il fit in modo significativo, quasi a 4\sigma. Però bisogna stare attenti a come il modello usa questa libertà. Nel caso in cui lasci pollin sia sulla reflection sia sulla Comptonizzazione, il fit trova una soluzione formalmente buona, ma fisicamente poco convincente: la slope della reflection diventa enorme, e quindi il PD intrinseco della reflection sale a valori mostruosi tra 6 e 8 keV. Il fatto che, imponendo un angolo comune, la slope della reflection crolli e diventi compatibile con zero mentre quella della Comptonizzazione resta positiva è molto istruttivo. Ti sta dicendo che il dato non richiede affatto in modo robusto una reflection fortemente crescente; lo fa solo quando le dai abbastanza libertà da assorbire su di lei quasi tutta la crescita della PD totale.

Secondo me questo è uno dei punti centrali della discussione. Il modello con due pollin non va letto come misura della PD della reflection, ma come dimostrazione di una degeneracy: se entrambe le componenti sono troppo libere, il fit può scaricare la crescita osservata sulla reflection, anche se questa pesa poco in flusso. E infatti i parametri che ottieni sono proprio quelli tipici di una soluzione matematicamente possibile ma fisicamente sospetta. Il fatto che la PA della reflection venga anche molto diversa, e molto più incerta, rispetto a quella della componente Comptonizzata, rafforza l’idea che la reflection non sia davvero ben vincolata dai dati.

Per questo i modelli misti mi sembrano più interessanti dei modelli completamente simmetrici. Il caso con reflection a PD costante e Comptonizzazione con pollin è, a mio avviso, il più sobrio e uno dei più credibili. Il fit resta molto buono, la crescita della PD è riprodotta, e soprattutto non sei costretto a spingere la reflection a polarizzazioni irreali. Il fatto che, legando anche gli angoli, il \chi^2 peggiori solo di pochissimo indica che non c’è vera evidenza di PA diverse tra reflection e continuo. In altre parole: il quadro minimo che i dati sembrano preferire è una componente dominante, con PA circa costante, la cui PD cresce moderatamente con l’energia; la reflection può contribuire, ma non serve che abbia una dipendenza estrema.

Viceversa, il caso opposto, cioè pollin sulla reflection e polconst sulla Comptonizzazione, continua a darti fit formalmente buoni ma al prezzo di una reflection assurda. E il polpow sulla reflection è ancora peggio, perché spinge il PD intrinseco a saturare o superare il 100\% alle alte energie. Il fatto che il \chi^2 sia sostanzialmente indistinguibile dal caso misto o dal caso con crescita della Comptonizzazione è, per me, la prova definitiva che quei modelli non stanno misurando la fisica della reflection, ma solo sfruttando una libertà parametrica per descrivere un andamento globale.

Quindi io, discutendoli, direi così. I dati con la DU2 rafforzano in modo robusto il risultato model-independent che la PD totale cresce con l’energia mentre la PA resta costante. Quando si tenta una decomposizione per componenti, più configurazioni riescono a descrivere i dati in modo comparabile, ma i modelli in cui la crescita è attribuita principalmente alla reflection richiedono spesso polarizzazioni intrinseche troppo elevate per essere considerate affidabili. Al contrario, una descrizione in cui la reflection ha una polarizzazione costante o debolmente variabile, mentre la componente Comptonizzata mostra un aumento moderato con l’energia, fornisce un fit ugualmente buono ma fisicamente molto più plausibile. Questo suggerisce che i dati richiedano con sicurezza una crescita della polarizzazione totale, ma non consentano ancora di identificare in modo univoco quale componente ne sia responsabile.

Se vuoi il mio parere secco, la narrativa più forte è questa: prima mostri Model A contro Model B come risultato principale; poi fai vedere che la decomposizione in componenti è degenerata; infine dici che, tra le soluzioni possibili, quelle che lasciano crescere troppo la reflection portano a valori non fisici, mentre i casi con reflection costante e crescita moderata della Comptonizzazione sono i più ragionevoli. Questa, secondo me, è una discussione molto solida e difficilmente attaccabile.
----

Io, per il paper, preferirei i due PA collegati, a meno che tu non abbia un miglioramento statisticamente chiaro e fisicamente leggibile lasciandoli liberi.
Il motivo non è solo “tenere il modello semplice”, ma proprio quello che mostrano i tuoi fit. Quando li lasci liberi, la PA della componente dominante resta sempre vicina alla PA totale, mentre quella della reflection tende a essere molto più incerta e instabile. Questo suggerisce che i dati non stanno davvero misurando due assi geometrici distinti. Stanno soprattutto misurando un unico asse dominante, e il resto viene assorbito dalla degeneracy della componente più debole. In queste condizioni, lasciare due PA liberi rischia di dare l’illusione di una struttura più complessa di quella che i dati possono davvero sostenere.
Quindi io la imposterei così: il modello di riferimento è quello con PA comune, perché non c’è evidenza robusta di una rotazione della PA con l’energia, e neppure una necessità statistica forte di due angoli distinti. Poi, magari, puoi dire che hai verificato anche il caso con PA liberi e che i risultati non cambiano in modo sostanziale, mentre la PA della reflection resta poco vincolata. Questo ti mette al riparo da obiezioni del referee del tipo “avete provato a lasciarli liberi?”.

Sul secondo punto, sì: questa è esattamente la giustificazione giusta per una reflection a PD costante.
Non devi dire che fisicamente ti aspetti una reflection davvero costante. Anzi, puoi dire apertamente il contrario: i modelli teorici di riflessione polarizzata, incluso il lavoro di Podgorný, indicano che la PD della reflection può variare con l’energia e spesso crescere in 2–8 keV. Però, nel tuo dataset, la reflection contribuisce relativamente poco al flusso totale nella banda IXPE, specialmente alle energie più alte. Questo significa che la sua dipendenza energetica non è ben vincolata dai dati. Quando la lasci libera, il fit tende a spingerla verso valori estremi e poco plausibili; quindi il dato non sta realmente misurando la sua forma energetica, sta solo sfruttando quella libertà per descrivere la crescita della PD totale.
Per questo una reflection a PD costante si può giustificare molto bene come approssimazione fenomenologica. In sostanza stai dicendo: sappiamo che in principio la reflection può essere variabile, ma nel nostro caso la sua frazione di flusso è troppo piccola per permettere una misura affidabile di tale variazione. Di conseguenza, la trattiamo come costante per evitare che il fit attribuisca artificialmente a questa componente una crescita estrema non realmente richiesta dai dati.
Questa è una giustificazione molto solida, e secondo me va proprio esplicitata così. Non è “assumiamo che sia costante perché lo crediamo fisicamente”, ma “la assumiamo costante perché i dati non ne vincolano robustamente la dipendenza energetica, e questa scelta evita soluzioni non fisiche”.
We also tested models in which the reflection and Comptonized components were allowed to have independent polarization angles. However, this did not lead to a qualitatively different solution, while the polarization angle of the reflection component remained poorly constrained. Since no significant rotation of the observed PA with energy is detected, we adopted a common PA as our reference configuration.

In addition, although the intrinsic polarization of the reflected component is expected to vary with energy in principle, its flux contribution in the IXPE band is relatively small, especially at the highest energies. As a consequence, the data do not constrain its energy dependence robustly. When the reflection PD is left free to increase with energy, the fits tend to drive it toward unrealistically large values, indicating a strong degeneracy rather than a reliable physical measurement. For this reason, we regard a constant reflection polarization as a conservative phenomenological approximation, while the observed increase of the total PD is more naturally accounted for by the dominant Comptonized component.
